Plug-and-Play Priors for Reconstruction-based Placental Image Registration

This paper presents a novel deformable registration framework, leveraging an image prior specified through a denoising function, for severely noise-corrupted placental images. Recent work on plug-and-play (PnP) priors has shown the state-of-the-art performance of reconstruction algorithms under such priors in a range of imaging applications. Integration of powerful image denoisers into advanced registration methods provides our model with a flexibility to accommodate datasets that have low signal-to-noise ratios (SNRs). We demonstrate the performance of our method under a wide variety of denoising models in the context of diffeomorphic image registration. Experimental results show that our model substantially improves the accuracy of spatial alignment in applications of 3D in-utero diffusion-weighted MR images (DW-MRI) that suffer from low SNR and large spatial transformations.

==> recycle/algorithm.tex <==
\section{Plug-and-Play Priors}
\subsection{Joint Objective Function}
\paragraph{Joint optimization objective function}
\begin{align} 
    \hat{I}, \hat{\Phi} &= \argmin_{I, \Phi}{ \frac{1}{2}\left \| I - I_T \right \|_2^2  + 
                            \lambda_{TV}TV(I) +
                            \lambda_{reg}R(\Phi) +
                            \frac{\rho}{2}\left \| I - I_S(\Phi) \right \|_2^2
                            }
\end{align}

\subsection{Alternating optimization objective function}
\begin{align} 
    \hat{I} 
    &= \argmin_{I}{ \frac{1}{2}\left \| I - \frac{1}{1+\rho}(I_T+\rho I_S(\Phi)) \right \|_2^2  + 
                            \frac{\lambda_{TV}}{1+\rho} TV(I)} \\
    \hat{\Phi}
    &= \argmin_{\Phi}{ \frac{\rho}{2\lambda_{reg}}\left \| I - I_S(\Phi) \right \|_2^2  + R(\Phi)}
\end{align}

If we note:
\begin{align}
    \tau &= \frac{\lambda_{TV}}{1+\rho} \\
    \frac{1}{2\sigma^2} &= \frac{\rho}{2\labmda_{reg}}
\end{align}

Then the objective functions can be rewritten as:
\begin{align}
    \hat{I}, \hat{\Phi} 
    &= \argmin_{I, \Phi}{ \frac{1}{2}\left \| I - I_T \right \|_2^2  + 
                            \tau(1+\rho)TV(I) +
                            \rho\sigma^2R(\Phi) +
                            \frac{\rho}{2}\left \| I - I_S(\Phi) \right \|_2^2
                            }\\
    \hat{I} 
    &= \argmin_{I}{ \frac{1}{2}\left \| I - \frac{1}{1+\rho}(I_T+\rho I_S(\Phi)) \right \|_2^2  + 
                            \tau TV(I)}\\
    \hat{\Phi}
    &= \argmin_{\Phi}{ \frac{1}{2\sigma^2}\left \| I - I_S(\Phi) \right \|_2^2  + R(\Phi)}
\end{align}

\subsection{Derivation of TV denoising objective function}
\begin{align} 
    L&(I, \Phi) \\
    &= { \frac{1}{2}\left \| I - I_T \right \|_2^2  + 
                            \lambda_{TV}TV(I) +
                            \lambda_{reg}R(\Phi) +
                            \frac{\rho}{2}\left \| I - I_S(\Phi) \right \|_2^2
                            }\\
    &= L_1 + L_2\\
    L_1&(I, \Phi) \\
    &= { \frac{1}{2}\left \| I - I_T \right \|_2^2  + 
                            \frac{\rho}{2}\left \| I - I_S(\Phi) \right \|_2^2
                            }\\
    &= \frac{1}{2}(I-I_T)^T(I-I_T) + \frac{\rho}{2}(I-I_S(\Phi))^T(I-I_S(\Phi))\\
    &= \frac{1}{2}(I^T-I_T^T)(I-I_T) + \frac{\rho}{2}(I^T-I_S(\Phi)^T)(I-I_S(\Phi))\\
    &= \frac{1}{2}(I^TI-2I_T^TI + I_T^TI_T) + \frac{\rho}{2}(I^TI-2I_S(\Phi)^TI + I_S(\Phi)^TI_S(\Phi))\\
    &= \frac{1+\rho}{2}I^TI - (I_T^T+\rho I_S(\Phi)^T)I + \frac{1}{2}I_T^TI_T + \frac{1}{2}I_S(\Phi)^TI_S(\Phi)\\
    &= \frac{1}{2}{\left( (1+\rho)\left \| I - \frac{1}{1+\rho}(I_T + \rho I_S(\phi)) \right \|_2^2 
                        - \frac{1}{\sqrt{1+\rho}}\left \| I_T + (1+\rho)I_S(\phi) \right \|_2^2
                        + \left \| I_T \right \|_2^2 
                        + \rho\left \| I_S(\phi) \right \|_2^2 
                        \right)}\\
    L_2(I, \phi) \\
    &= \lambda_{TV}TV(I) + \lambda_{reg}R(\Phi)
\end{align}
Therefore,
\begin{align}
    \hat{I} &= \argmin_I L(I) \\
            &= \argmin_I (1+\rho)\left \| I - \frac{1}{1+\rho}(I_T + \rho I_S(\phi)) \right \|_2^2 + \lambda_{TV}TV(I)\\
            &= { \frac{1}{2}\left \| I - \frac{1}{1+\rho}(I_T+\rho I_S(\Phi)) \right \|_2^2  + 
                            \frac{\lambda_{TV}}{1+\rho} TV(I)}
\end{align}

==> sections/2-Background/pnp.tex <==
Based on proximal methods such as FISTA and ADMM, the idea of Plug-and-play (PnP) priors is introduced in \cite{venkatakrishnan2013plug} to solve image reconstruction problems with the help of existing denoising algorithms. Consider the general image reconstruction problem:
$\hat{x} = \underset{x}{\mathrm{argmin}}{\;\text{dist}(x, x_0) + \tau \text{reg}(x)}$, where $x_0$ is the observation, $\text{dist}(x)$ is the data fidelity term, $\text{reg}(x)$ is the regularization term and $\tau$ is the weight parameter. As many popular regularizers are not differentiable, gradient-based optimization cannot be used in these cases. Instead, assuming $\text{dist}(x)$ is differentiable and $\text{reg}(x)$ is indifferentiable, the well-studied FISTA solves the optimization task by following these steps:
\begin{subequations}
\begin{align}
\label{eq:FISTA-S1}
z^t &\leftarrow s^{t-1} - \gamma \nabla \text{dist}(s^{t-1}, x_0) \\
\label{eq:FISTA-S2}
x_t &\leftarrow \text{prox}_{\gamma\tau R}(z^t) \\
\label{eq:FISTA-S3}
q_t &\leftarrow \frac{1}{2}\left( 1+ \sqrt{1+4q^2_{t-1}} \right) \\
\label{eq:FISTA-S4}
s^t &\leftarrow x^t + \left(  (q_{t-1} - 1)/q_t \right)(x^t - x^{t-1})
\end{align}
\end{subequations}
for $t=1,2,...$ where $q_0=1$ and $x^0=s^0=x_{\text{init}}\in\mathbb{R}^N$.  $\gamma$ is the step-size parameter, of which the setting strategies can be found in \cite{ochs2014ipiano}, and $\{q_t\}_{t\in\mathbb{N}}$ are the parameters used in (\ref{eq:FISTA-S4}) to improve the convergence rate \cite{beck2009fast}. The proximal operator in (\ref{eq:FISTA-S2}) is defined as:
\begin{equation}
    \text{prox}_{\gamma\tauR}(z) \triangleq \argmin_{x\in\mathbb{R}^N}\left\{ \frac{1}{2}\left\| x-z \right\|_{l_2}^2 + \tau \text{reg}(x) \right\}
  \label{eq:proximal}
\end{equation}
It can be easily noticed that (\ref{eq:proximal}) has the same form as an image denoising problem with regularization term $R$. And the core idea of PnP prior is that we can replace the proximal operator in (\ref{eq:FISTA-S2}) with an arbitrary image denoisier $\text{D}_\sigma$, i.e. $x_t\leftarrow\text{D}_{\sigma}(z^t)$, where the strength parameter $\sigma \triangleq \sqrt{\gamma\tau}$. For optimization-based denoising such as TV denoising, it is equal to replace $\text{reg}(x)$ with TV regularizer $\left\| x \right\|_{l1}$. For other kinds of denoisers such as BM3D, however, it is equal to replace $\text{reg}(x)$ with some potential prior term, which we refer as PnP prior. Although PnP prior is less interpretable and the convergence of PnP-based algorithms is not guaranteed, it is shown to be rather effective \cite{kamilov2017plug}.

==> sections/2-Background/reconstruction.tex <==
\subsection{Image Reconstruction}
As is discussed in previous sections, image reconstruction is necessary for improving image quality to aid registration, and it's a natural choice to use denoising algorithms. There are many kinds of denoising algorithms. Optimization-based denoising algorithms, such as total variation (TV) denoising, are widely used in medical image processing tasks. Similar to the image registration algorithms we introduced in last section, it also models the task as a optimizing an objective function, which includes the dissimilarity term and often the regularization term. Denoising algorithms, however, usually search for a denoised image instead of a denoising transformation:
$\hat{I} = \underset{I}{\mathrm{argmin}} \;\mathrm{dist}(I, I_0) + \mathrm{reg}(I),$
where $I_0$ is the observed noisy image and $\hat{I}$ is the denoised image. For example, in TV denoising algorithm $\text{dist}(\cdot, \cdot)$ is set to be the sum-of-squared difference, and $\text{reg}(I)=\left\|I\right\|_1$ 

There are also denoising methods that cannot be presented as a optimization task such as . For example, non-local mean (NLM)\cite{buades2005non} algorithm works by taking similar image blocks and taking the averaging as local denoising result. Another example, block-matching and 3D filtering (BM3D)\cite{dabov2007video} algorithm, which collects matching blocks and denoises by 3D filtering in Fourier space. 


% \begin{itemize}
%     \item Image reconstruction
%     \item Why denoising algorithms
%     \item Introduction to denoising algorithms used in this work
% \end{itemize}

% As is discussed in the introduction, image reconstruction is necessary for improving image quality and thus aiding registration. And it should be stated clear that here "reconstruction algorithms" refers to only the algorithms applied on images to improve their visual effect, such as image denoising and super-resolution, but not the process to generate images from raw signal collected in CT or MRI machine. 

% Since the problem is the low image quality, using image denoising algorithms is a natural choice, and the question is which algorithm should we use. Optimization-based denoising algorithms, such as total variation (TV) denoising, are widely used in medical image processing tasks. Similar to the image registration algorithms we introduced in last section, it also models the task as a optimizing an objective function, which includes the dissimilarity term and often the regularization term. Denoising algorithms, however, usually search for a denoised image instead of a denoising transformation:
% \begin{equation}
%     \hat{I} = \argmin_{I} \mathrm{dist}(I, I_0) + \mathrm{reg}(I),
% \label{eq:denoising-general}
% \end{equation}
% where $I_0$ is the observed noisy image and $\hat{I}$ is the denoised image. In TV denoising algorithm, $\text{dist}(\cdot, 
% \cdot)$ is set to be the sum-of-squared difference, and $\text{reg}(I)=\left\|I\right\|_1$ 

% As is discussed in the introduction, there are also denoising methods that cannot be presented as a optimization task. For example, non-local mean (NLM)\cite{buades2005non} algorithm works by taking similar image blocks and taking the averaging as local denoising result. Another example, block-matching and 3D filtering (BM3D)\cite{dabov2007video} algorithm, somehow works. 


% Search-based. Non-local mean and BM3D. -- which cannot be used in joint optimization methods.

% Here we want to discuss about neural network based methods. 

% Neural network. On one hand, cannot use pretrained which help amount of data. On the other hand, possible to joint optimization but no related work and no guarantee. 
